The AAAtrig algorithm for rational approximation of periodic functions

We present an extension of the AAA (adaptive Antoulas--Anderson) algorithm for periodic functions, called 'AAAtrig'. The algorithm uses the key steps of AAA approximation by (i) representing the approximant in (trigonometric) barycentric form and (ii) selecting the support points greedily. Accordingly, AAAtrig inherits all the favourable characteristics of AAA and is thus extremely flexible and robust, being able to consider quite general sets of sample points in the complex plane. We consider a range of applications with particular emphasis on solving Laplace's equation in periodic domains and compressing periodic conformal maps. These results reproduce the tapered exponential clustering effect observed in other recent studies. The algorithm is implemented in Chebfun.

==> sections/specialsupport.tex <==
\subsubsection{Special case: $\pi$ is a support point} \label{Sec:specialSupport}
%
\newcommand{\pSum}{\sum_{j=2}^m}
We now consider the special case where the number of support points is odd, and
$z_k = \pi$ is a support point for some $k$.
For simplicity, we take $k=1$ so that $z_1 = \pi$.
The approximant \eqref{Eq:trigApproxEven} may therefore be rewritten as 
%
\begin{align*}
r(z) =  \Bigg( -f_1 w_1 \tan\left(\frac{z}{2} \right) +
& \pSum f_j w_j \cot \left(\frac{z - z_j}{2}\right) \Bigg) \Bigg/\\
 \Bigg(  - w_1 \tan\left(\frac{z}{2} \right) + 
&\pSum w_j \cot \left(\frac{z - z_j}{2}\right) \Bigg) .
\end{align*}
%
Now applying the transformation \eqref{Eq:trans} yields
%
\begin{align}
	r(z) \triangleq R(\tilde{z})= \left. \left( \frac{c_n}{\tilde{z}} - f_1 w_1 +
	\pSum \frac{f_j \tilde{w}_j}{\tilde{z}(\tilde{z} - \tilde{z}_j)} \right)\middle/
	\left(\frac{c_d}{\tilde{z}} - w_1 + 
	\pSum \frac{\tilde{w}_j}{\tilde{z}(\tilde{z} - \tilde{z}_j)} \right)\right. \label{Eq:specialR}
\end{align}
%
where $c_n$ and $c_d$ are defined in \eqref{Eq:constDef} with the exception that the
first term is now excluded in the summation. 
Finding the poles and zeros of \eqref{Eq:specialR} can now be formulated as a general eigenvalue problem.
For example, the zeros of \eqref{Eq:specialR} are the eigenvalues of the problem
%
\begin{align}
	\begin{pmatrix}
		-f_1 w_1 & c_d & f_2 \tilde{w_2} &\cdots & f_m \tilde{w}_m\\
		1 &0 &&&\\
	0 & 1& \tilde{z}_2 &\\
	\vdots & \vdots&& \ddots \\
	0 & 1 &&&\tilde{z}_m
	\end{pmatrix} \boldsymbol{v} = \lambda
	\begin{pmatrix}
		0 & & & &\\
		  & 1 & & &\\
		  & & \ddots & &\\
	& & & \ddots &\\
	& & & & 1
	\end{pmatrix}
	\boldsymbol{v}
\end{align}
%
which has eigenvectors
%
\begin{align*}
	\boldsymbol{v} = \left[1 , \frac{1}{\lambda}, 
	\frac{1}{\lambda(\lambda - \tilde{z}_2)},\cdots, \frac{1}{\lambda(\lambda - \tilde{z}_m)} \right]^{T}.
\end{align*}
%
The poles can be found in a similar manner.
\iffalse
 $\tilde{z}_0$ replaced by $0$, $\tilde{w_j}$ For example, the poles of $R$ are the eigenvalues of the generalised eigenvalue problem
%
\begin{align}
\begin{pmatrix}
\hat{c}_d & \hat{A}_d &\tilde{w}_1 & \cdots & \tilde{w}_m\\
1 & 0&&&\\
\vdots & & \tilde{z}_2 &&\\
 &&&\ddots&\\
1 &&&&\tilde{z}_m
\end{pmatrix} \boldsymbol{v} = \lambda
\begin{pmatrix}
0 & & &\\
& 1 & &\\
& & \ddots &\\
& & & 1
\end{pmatrix}
\boldsymbol{v} 
\end{align}
%

are the poles of $R$, and the eigenvectors are given by
%
\begin{align*}
\boldsymbol{v} = \left[1 , 1/(\lambda - \tilde{z}_1),\cdots, 1/(\lambda - \tilde{z}_m) \right]^{T}.
\end{align*}
\fi
%


==> sections/spectral-method.tex <==
\subsection{Differentiating the approximant}
%
One advantage of the barycentric representation adopted in this paper is the straightforward evaluation of derivatives
using differentiation matrices, thereby avoiding repeated application of the quotient rule \cite{Tee2006}.
The $p$-th order differentiation matrix is the $m\times m$ matrix $\bD^{(p)}$ such
that if $f$ is a vector of function values associated with the grid $\{z_j\}$ then
$\bD^{(p)} \bfun$ is the vector obtained by interpolating these data and then differentiating the interpolant $p$ times
and evaluating at the grid points. 
The differentiation matrices for rational trigonometric barycentric forms were derived by Baltensperger 
\cite{Baltensperger2002} as
%
\begin{align*}
	D_{jk}^{(1)} &=
	\begin{dcases}
		\frac{1}{2} \cdot \frac{w_k}{w_j} \cdot \cst\left( \frac{z_j - z_k}{2}  \right),
	 	& \textrm{if } j \neq k, \\
		- \sum_{i=0, i \neq j}^{n-1}D_{ji}^{(1)},
	 	& \textrm{if } j = k.
	\end{dcases}
\end{align*}
%
Recurrence relations for higher-order differentiation matrices are also given by \cite{Baltensperger2002}.
The off-diagonal entries for the differentiation matrix are given by
%
\begin{align}
	D_{jk}^{(p)}= 
	\cst\left( \frac{z_j - z_k}{2} \right) 
	\sum_{q=1}^{p} {p \choose q} \Bigg[\frac{w_k}{w_j} D_{jj}^{(p-q)}
		    &	\partial_\xi^{(q)}
			\cst^{-1} \left( \frac{\xi - z_j}{2} \right) \Bigg|_{\xi = z_j} \\
					- D_{jk}^{(p-q)}
		    &\partial_\xi^{(q)}
			\cst^{-1} \left( \frac{\xi - z_k}{2} \right) \Bigg|_{\xi = z_j} 
		\Bigg]	
\end{align}
%
whilst the diagonal entries are given by
%
\begin{align}
	D_{jj}^{(p)} = - \sum_{\substack{k=0\\k\neq j}}^{m-1} D_{jk}^{(p)}, 
\end{align}
%
The superscript $-1$ here refers to the reciprocal of $\cst$ as opposed to the inverse function.

Differentiation away from a support point can be calculated with the recurrence relation
%
\begin{align}
	 r^{(p)}(z) &= \dfrac{\sum_{q = 0}^{p-1} {p \choose q} 
	 	\sum_{j=1}^{m} w_j \partial_z^{(p-q)} \cst \left( \frac{z - z_j}{2} \right) 
	\partial_z^{(q)} \left(f_j - r(z)\right) }
 {\sum_{j=1}^{m} w_j \cst \left( \frac{z - z_j}{2} \right)} .
\end{align}
%
The derivatives of $\cst$ and $\cst^{-1}$ can be rapidly computed with the relevant derivative
polynomials \cite{Hoffman1995}.
%Expressions for the higher-order derivatives of $\cst$ and $\cst^{-1}$ quickly become unwieldy
%Fortunately, more compact forms are available.
%The $p$-tkh derivative of the cotangent may be written as
%%
%\begin{align*}
%	\partial^{(p)} \cot(z) = \frac{Q_p(\cos(z))}{\sin^{p+1}(z)} 
%\end{align*}
%%
%where the $Q_p$ are polynomials defined by the recursion relation
%%
%\begin{align*}
%	Q_0(x) = x, \qquad
%	Q_{p+1}(x)= -((p+1) x Q_p(x) + (1-x^2) Q_p^\prime (x)).
%\end{align*}
%%
%%First, Euler's reflection formula yields
%%\eqref{Eq:ML} shows that that the cotangent may be expressed in terms of the digamma function as
%%%
%%\begin{align}
%%	\cot(z) &= \frac{1}{\pi} \left( \psi\left(1 - \frac{z}{\pi} \right) - \psi\left( \frac{z}{\pi} \right) \right)
%%\end{align}
%%%
%%where
%%%
%%\begin{align}
%%	\psi(s + 1) &= -\gamma + \sum_{k=1}^\infty \left( \frac{1}{k} - \frac{1}{k+s}  \right).
%%\end{align}
%%%
%%Accordingly, the $q$-th derivative of the cotangent is expressible as
%%%
%%\begin{align}
%%	\partial_z^{(q)}\cot(z) &=
%%	\frac{1}{\pi^{q+1}} \left( (-1)^q \psi^{(q)} \left(1 - \frac{z}{\pi} \right) - \psi^{(q)}\left( \frac{z}{\pi} \right) \right)
%%\end{align}
%%
%The higher-order derivatives of the other representations of $\cst$ and $\cst^{-1}$ follow from
%%
%\begin{align*}
%	\csc(z) &= \cot \left( \frac{z}{2} \right) - \cot(z), \qquad \tan(z) = -\cot\left(z - \frac{\pi}{2} \right).
%\end{align*}
%%


==> sections/summary.tex <==
%\subsection{Summary}
%%
%The AAAtrig algorithm and subroutines can be summarised in the following pseudocode:
% \begin{algorithm}
% 	\caption{Pseudocode for the AAATrig algorithm and subroutines}
% \begin{algorithmic}
% 	\Procedure{AAATrig}{}
% 	\State Project all the sample points onto the strip $0\leq\Re[z_j]<2 \pi$
% \State Set $m=0$, error $=\infty$
% \While{error $>$ tolerance}
% \State{Update $m$\texttt{++}}
% \State{Define the reduced sample sets $Z^{(m)} = Z \setminus \{z_1, \cdots, z_m\}$, $F^{(m)} = f(Z^{(m)})$}
% \State{Find the sample point with the maximum residual error}
% \State{Add this sample point to the set of support points}
% \State{Find the weights that solve the least-squares problem}
% \State{Calculate the new error}
% \EndWhile
% \EndProcedure
% \Procedure{przTrig}{}
% \State Calculate the poles, residues and zeros according to section \ref{Sec:polesZeros}
% \EndProcedure
% \Procedure{cleanupTrig}{}
% \For{each pole with sufficiently small residue}
% \State remove the support point closest to that pole
% \EndFor
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

